The Continuous-Time RC-Chain ADC

An amplifier-less continuous-time analog-to-digital converter consisting of only passives, comparators, and inverters is presented. Beyond simplicity, the architecture displays significant robustness properties with respect to component variations and comparator input offsets. We give an analytical design procedure demonstrating how to parameterize the architecture to a range of signal-to-noise and bandwidth requirements and validate the procedure's accuracy with behavioral transient simulations.

==> tex/acronyms.tex <==
\begin{acronym}
    \acro{AGDA}{analog-gain digital-attenuation ratio}
    \acro{CBADC}[CB-ADC]{control-bounded analog-to-digital converter}
    % \acro{CTSDM}{continuous-time sigma-delta modulator}
    \acro{CTSDM}[CT-$\Sigma\Delta$M]{continuous-time sigma-delta modulator}
    \acro{CTSD}[CT-$\Sigma\Delta$]{continuous-time sigma-delta}
    \acro{SDM}[$\Sigma\Delta$M]{sigma-delta modulator}
    \acro{CTP}{continuous-time pipeline}
    \acro{DTSDM}{discrete-time sigma-delta modulator}
    \acro{CRFB}{cascade of resonators with feedback}
    \acro{CRFF}{cascade of resonators with feedforward}

    \acro{CTADC}[CT-ADC]{continuous-time analog-to-digital converter}
    \acro{DTADC}[DT-ADC]{discrete-time analog-to-digital converter}

    \acro{ENOB}{effective number of bits}
    \acro{SNR}{signal-to-noise ratio}
    \acro{SNDR}{signal-to-noise-and-distortion ratio}
    \acro{SQNR}{signal-to-quantization-noise ratio}
    \acro{SC}{switched-capacitor}
    \acro{CT}{continuous-time}
    \acro{DT}{discrete-time}
    \acro{PSD}{power spectral density}

    \acro{NTF}{noise transfer function}
    \acro{STF}{signal transfer function}

    \acro{CI}{chain-of-integrators}
    \acro{LF}{leapfrog}
    \acro{DC}{digital control}
    \acro{AS}{analog system}
    \acro{DE}{digital estimator}

    \acro{RZ}{return-to-zero}
    \acro{NRZ}{non-return-to-zero}
    \acro{SCR}{switched-capacitor-resistor}
    \acro{DAC}{digital-to-analog converter}
    \acro{ADC}{analog-to-digital converter}

    \acro{FIR}{finite impulse response}
    \acro{FS}{full scale}
    \acro{OSR}{oversampling ratio}
    \acro{OTA}{operational transconductance amplifier}
    \acro{PLL}{phase-locked loop}
    \acro{VCO}{voltage-controlled oscillator}
    \acro{PM}{phase-modulated}
    \acro{FM}{frequency-modulated}

    \acro{CIC}{cascaded integrator–comb filter}
    \acro{GBWP}{gain-bandwidth product}

    \acro{SAR}{successive approximation register}
    \acro{FS}{full-scale}
    \acro{dB}{decibel}
    \acro{BW}{bandwidth}
    \acro{RMS}{root mean square}
    \acro{IC}{integrated circuit}

\end{acronym}
